Short-term traffic prediction using physics-aware neural networks

In this work, we propose an algorithm performing short-term predictions of the flux of vehicles on a stretch of road, using past measurements of the flux. This algorithm is based on a physics-aware recurrent neural network. A discretization of a macroscopic traffic flow model (using the so-called Traffic Reaction Model) is embedded in the architecture of the network and yields flux predictions based on estimated and predicted space-time dependent traffic parameters. These parameters are themselves obtained using a succession of LSTM ans simple recurrent neural networks. Besides, on top of the predictions, the algorithm yields a smoothing of its inputs which is also physically-constrained by the macroscopic traffic flow model. The algorithm is tested on raw flux measurements obtained from loop detectors.

==> fig/RMSE_Compar_Obs.tex <==
\begin{tabular}{*{3}{C{2cm}}}
\toprule
{} &  TRM Prediction &  Last known state \\ \midrule
$N_f=3$ &        3.84e-01 &          5.29e-01 \\ \hline
$N_f=5$ &        4.20e-01 &          5.45e-01 \\ \bottomrule
\end{tabular}


==> fig/RMSE_Compar_Obs_Unobs.tex <==
\begin{tabular}{*{3}{C{2cm}}}
\toprule
{} &  On obseved cells &  On hidden cells \\ \midrule
$N_f=3$ &          3.84e-01 &         3.95e-01 \\ \hline
$N_f=5$ &          4.20e-01 &         4.11e-01 \\ \bottomrule
\end{tabular}


==> fig/RMSE_Smooth_Compar.tex <==
\begin{tabular}{*{3}{C{2cm}}}
\toprule
{} &  $N_f=3$ &  $N_f=5$ \\ \midrule
$N_f=3$ &        0 & 1.27e-01 \\ \hline
$N_f=5$ & 1.27e-01 &        0 \\ \bottomrule
\end{tabular}

